Graph Propagation Transformer for Graph Representation Learning

This paper presents a novel transformer architecture for graph representation learning. The core insight of our method is to fully consider the information propagation among nodes and edges in a graph when building the attention module in the transformer blocks. Specifically, we propose a new attention mechanism called Graph Propagation Attention (GPA). It explicitly passes the information among nodes and edges in three ways, i.e. node-to-node, node-to-edge, and edge-to-node, which is essential for learning graph-structured data. On this basis, we design an effective transformer architecture named Graph Propagation Transformer (GPTrans) to further help learn graph data. We verify the performance of GPTrans in a wide range of graph learning experiments on several benchmark datasets. These results show that our method outperforms many state-of-the-art transformer-based graph models with better performance. The code will be released at https://github.com/czczup/GPTrans.

==> tables/configurations.tex <==
\begin{tabular}{l|c}
    \toprule
    Hyper-parameter
        & GPTrans-T/S/B/L \\
    \midrule
    weight init
        & \\
    optimizer
        & \\
    base learning rate
        & \\
    weight decay
        & \\
    optimizer momentum
        & \\
    batch size
        & \\
    training epochs
        & \\
    learning rate schedule
        & \\
    warmup schedule
        & \\
    TBA
        & \\
    \bottomrule
\end{tabular}

==> tables/datasets.tex <==
\begin{tabular}{l|c|c|c|c|c}
    \toprule
    Dataset
        & \#Graphs 
        & Avg. Nodes
        & Avg. Edges
        & Task Type
        & Metric \\
    \midrule
    % \multicolumn{6}{l}{\emph{Graph-level Tasks}} \\
    PCQM4M~\cite{hu2021ogb}
        & 3,803,453 % #Graphs
        & 14.1 % Avg. Nodes
        & 14.6 % Avg. Edges
        & Graph Regression % Task Type
        & Mean Absolute Error \\ % Metric
    PCQM4Mv2~\cite{hu2021ogb}
        & 3,746,619 % #Graphs
        & 14.1 % Avg. Nodes
        & 14.6 % Avg. Edges
        & Graph Regression % Task Type
        & Mean Absolute Error \\ % Metric
    MolHIV~\cite{hu2021ogb}
        & 41,127 % #Graphs
        & 25.5 % Avg. Nodes, 1,048,738/41,127
        & 27.5 % Avg. Edges, 1,130,993/41,127
        & Graph Classification % Task Type
        & ROC-AUC \\ % Metric
    MolPCBA~\cite{hu2021ogb}
        & 437,929 % #Graphs
        & 26.0 % Avg. Nodes, 11,386,154/437,929
        & 28.1 % Avg. Edges, 12,305,805/437,929
        & Graph Classification % Task Type
        & Average Precision \\ % Metric
    ZINC~\cite{dwivedi2020benchmarking}
        & 12,000 % #Graphs
        & 23.2 % Avg. Nodes
        & 49.8 % Avg. Edges
        & Graph Regression % Task Type
        & Mean Absolute Error \\ % Metric
    \midrule
    PATTERN~\cite{dwivedi2020benchmarking}
        & 14,000 % #Graphs
        & 117.5 % Avg. Nodes
        & 4749.2 % Avg. Edges
        & Node Classification % Task Type
        & Accuracy \\ % Metric
    CLUSTER~\cite{dwivedi2020benchmarking}     
        & 12,000 % #Graphs
        & 117.2 % Avg. Nodes
        & 4301.7 % Avg. Edges
        & Node Classification % Task Type
        & Accuracy \\ % Metric
    \midrule
    TSP~\cite{dwivedi2020benchmarking}
        & 12,000 % #Graphs
        & 275.6 % Avg. Nodes
        & 6894.0 % Avg. Edges
        & Edge Classification % Task Type
        & F1 Score \\ % Metric
    \bottomrule
\end{tabular}
\vspace{3em}

==> tables/models.tex <==
\begin{tabular}{l|c}
    \toprule
    Hyper-parameter
        & Nano/Tiny/Small/Base/Large \\
    \midrule
    \#Layers
        & 12/12/12/18/24 \\ % Large
    Dimension $d_1$
        & 80/256/384/608/736 \\ % Large
    Dimension $d_2$
        & 40/32/48/76/92 \\ % Large
     FFN Ratio $\alpha$
        & 1.0 \\ % Large
    \#Attention Head
        & 8/8/12/19/23 \\ % Large
    Dimension of Each Head
        & 10/32/32/32/32 \\ % Large
    Layer Scale & \no/\yes/\yes/\yes/\yes \\
    \bottomrule
\end{tabular}



==> tables/sup_params_ptn_clt_tsp.tex <==
\begin{tabular}{l|c|c|c}
    \toprule
    
        & \textbf{PATTERN} 
        & \textbf{CLUSTER} 
        & \textbf{TSP} \\
    \midrule\midrule
    Batch size 
        & 128 
        & 128 
        & 8 \\
    Number of epochs 
        & 200 
        & 200 
        & 200 \\
    % Reduce LR patience (epochs)
    %     & 10 
    %     & 10 
    %     & 5 \\
    % Number of layers, $L$ 
    %     &
    %     &
    %     & \\
    \bottomrule
\end{tabular}%

==> tables/training_mol.tex <==
\begin{tabular}{l|c|c}
    \toprule
    Dataset
        & MolHIV
        & MolPCBA \\
    Model
        & Base
        & Base/Large \\
    \midrule
    Initialization
        & PCQM4Mv2 
        & PCQM4Mv2 \\
    FFN Dropout
        & 0.1 %
        & 0.1/0.2 \\
    Embedding Dropout
        & 0.1
        & 0.1/0.2 \\ % Large
    Attention Dropout
        & 0.1
        & 0.1/0.2 \\
    Drop Path Rate 
        & 0.1
        & 0.1/0.4\\ 
    Max Epochs
        & 10  
        & 50  \\
    Peak Learning Rate
        & 2e-4
        & 4e-4 \\
    Min Learning Rete
        & 1e-4
        & 1e-9 \\
    Batch Size
        & 128
        & 128 \\
    Warm-up Epochs
        & 1 
        & 1 \\ % Large
    Learning Rate Decay
        & Cosine 
        & Cosine \\
    Adam $\epsilon$
        & 1e-8 
        & 1e-8\\
    Adam $(\beta_2, \beta_2)$
        & (0.9, 0.999)
        & (0.9, 0.999) \\
    Weight Decay 
        & 0.0 
        & 0.0 \\
    EMA
        & \yes
        & \yes \\
    \bottomrule
\end{tabular}

==> tables/training_others.tex <==
\begin{tabular}{l|c}
    \toprule
    Dataset
        & ZINC/PATTERN/CLUSTER/TSP \\
    \midrule
    FFN Dropout
        & 0.3 \\ % Large
    Embedding Dropout
        & 0.3 \\ % Large
    Attention Dropout
        & 0.5 \\ % Large
    Drop Path Rate 
        & 0.3 \\ % Large
    Max Epochs
        & 10000/1000/1000/1000  \\
    Peak Learning Rate
        & 5e-4 \\
    Batch Size
        & 256/256/256/32 \\ % Large
    Warm-up Epochs
        & 20 \\ % Large
    Learning Rate Decay
        & Cosine \\
    Weight Decay 
        & 0.05 \\
    EMA
        & \yes \\
    \bottomrule
\end{tabular}

==> tables/training_pcqm4m.tex <==

\begin{tabular}{l|ccccc}
    \toprule
    Hyper-parameter
        & Tiny/Small/Base/Large \\
    \midrule
    FFN Dropout
        & 0.1/0.1/0.1/0.2 \\ % Large
    Embedding Dropout
        & 0.1/0.1/0.1/0.2 \\ % Large
    Attention Dropout
        & 0.1/0.1/0.1/0.2 \\ % Large
    Drop Path Rate 
        & 0.1/0.1/0.2/0.4 \\ % Large
    Max Epochs
        & 300\\ % Large
    Warm-up Epochs
        & 20 \\ % Large
    Peak Learning Rate
        & 1e-3 \\ % Large
    Batch Size
        & 1024 \\ % Large
    Learning Rate Decay
        & Cosine \\
    Adam $\epsilon$
        & 1e-8 \\
    Adam $(\beta_2, \beta_2)$
        & (0.9, 0.999) \\
    Weight Decay 
        & 0.05 \\
    EMA
        & \yes \\
    \bottomrule
\end{tabular}

==> tables/zinc.tex <==
\begin{tabular}{l|cc}
    \toprule
    \textbf{Model} 
        & \textbf{\#Param} 
        & \textbf{Test MAE}$\downarrow$ \\
    \midrule
    \multicolumn{3}{l}{\emph{Non-transformer-based Methods}} \\
    GIN~\cite{xu2018powerful}
        & 510K
        & 0.526 $\pm$ 0.051 \\
    GraphSage (Hamilton et al. 2017)
        & 505K
        & 0.398 $\pm$ 0.002 \\
    GAT~\cite{velivckovic2017graph}
        & 531K
        & 0.384 $\pm$ 0.007 \\
    GCN~\cite{kipf2016semi}
        & 505K
        & 0.367 $\pm$ 0.011 \\
    GatedGCN-PE (Bresson et al. 2017)
        & 505K
        & 0.214 $\pm$ 0.006 \\
    PNA~\cite{corso2020principal}
        & 387K
        & 0.142 $\pm$ 0.010 \\
    \midrule
    \multicolumn{3}{l}{\emph{Transformer-based Methods}} \\
    GT~\cite{cai2020graph} 
        & 589K
        & 0.226 $\pm$ 0.014 \\
    SAN~\cite{kreuzer2021rethinking}
        & 509K 
        & 0.139 $\pm$ 0.006 \\
    Graphormer-Slim~\cite{ying2021graphormer}
        & 489K
        & 0.122 $\pm$ 0.006 \\
    GRPE-Small~\cite{park2022grpe}
        & 489K
        & 0.094 $\pm$ 0.002 \\
    EGT (Hussain et al. 2021)
        & 500K
        & 0.108 $\pm$ 0.009 \\
    \rowcolor{gray!20}
    GPTrans-Nano (ours) 
        & 504K
        & \textbf{0.102 $\pm$ 0.005}\\
    \bottomrule
\end{tabular}
